Reward Machines for Deep RL in Noisy and Uncertain Environments

Reward Machines provide an automaton-inspired structure for specifying instructions, safety constraints, and other temporally extended reward-worthy behaviour. By exposing the underlying structure of a reward function, they enable the decomposition of an RL task, leading to impressive gains in sample efficiency. Although Reward Machines and similar formal specifications have a rich history of application towards sequential decision-making problems, they critically rely on a ground-truth interpretation of the domain-specific vocabulary that forms the building blocks of the reward function--such ground-truth interpretations are elusive in the real world due in part to partial observability and noisy sensing. In this work, we explore the use of Reward Machines for Deep RL in noisy and uncertain environments. We characterize this problem as a POMDP and propose a suite of RL algorithms that exploit task structure under uncertain interpretation of the domain-specific vocabulary. Through theory and experiments, we expose pitfalls in naive approaches to this problem while simultaneously demonstrating how task structure can be successfully leveraged under noisy interpretations of the vocabulary.

==> sections/0-abstract.tex <==
\begin{abstract}

Formal languages, including Reward Machines and Linear Temporal Logic, provide effective mechanisms for specifying high-level instructions and exploiting task structure in deep Reinforcement Learning (RL). While formal languages have been widely adopted for a variety of sequential decision-making tasks, their use typically relies on a ground-truth interpretation of the symbols—the domain-specific vocabulary. In many practical applications, such ground-truth interpretations are difficult to specify or hard to evaluate due to partial observability or noisy sensing, and consequently, an RL agent may not faithfully interpret instructions or evaluate its progress towards completing those instructions. In this paper, we address this interpretation problem in the context of following temporally extended instructions specified by a Reward Machine. We characterize this problem as a Partially Observable Markov Decision Process and propose a suite of algorithms that leverage task structure under an uncertain symbolic interpretation. Experiments demonstrate the power and flexibility of our approach. \commental{I would like to highlight our contributions a bit better here if space permits.}

\end{abstract}


% Contributions:
% - We 




==> sections/0.5-new-abstract.tex <==
\begin{abstract}
Reward Machines provide an automata-inspired structure for specifying instructions, safety constraints, and other temporally extended reward-worthy behaviour. By exposing the underlying structure of acomplex reward function structure, they enable counterfactual learning updates, leading to that have resulted in impressive gains in sample efficiency gains. While Reward Machines have been employed in both tabular and deep RL settings, they have typically relied on a ground-truth interpretation of the domain-specific vocabulary that form the building blocks of the reward function. Such ground-truth interpretations can be elusive in many real-world settings, due in part to partial observability or noisy sensing. In this paper, we explore the use of Reward Machines for Deep RL in noisy and uncertain environments. We characterize this problem as a POMDP and propose a suite of RL algorithms that leverage task structure under uncertain interpretation of domain-specific vocabulary. Theoretical analysis exposes pitfalls in naive approaches to this problem, while experimental results show that our algorithms successfully leverage task structure to improve performance under noisy interpretations of the vocabulary. Our results provide a general framework for exploiting Reward Machines in partially observable environments.

\medskip
\textbf{Code and videos available at \url{https://github.com/andrewli77/reward-machines-noisy-environments}.}
\end{abstract}


==> sections/1-intro.tex <==
\section{Introduction}
\label{section:intro}

Formal languages (FLs) have long been used for objective specification in sequential decision-making domains. Using a set of domain-specific propositional variables, FLs like Linear Temporal Logic (LTL) \citep{pnueli1977temporal} can express rich temporal patterns---in our case, representing the desired objectives of an agent---by composing variables with temporal and logical operators. Such FLs offer unambiguous semantics while enabling formal procedures, including transformations to automata \citep{baier2008principles}, that expose a decision-making agent to the discrete structure underlying an objective. For these reasons, FLs have been adopted across a wide variety of domains, ranging from motion planning \citep{kress2009temporal, fainekos2009temporal, sun2024neurosymbolic} to robotic manipulation \citep{camacho2021reward,he2015towards, kunze2011logic} to, more recently, general deep Reinforcement Learning (RL) problems over large inputs \citep[e.g.,][]{aksaray2016q,li2017reinforcement,li2018policy, littman2017environment,icarte2018using,tor-etal-neurips19, hasanbeig2018logically,deeplcrl,alur2019,DBLP:conf/ijcai/0005T19,kuo2020encoding,HasanbeigKA20Deep,xu2020joint,xu2020active,furelos2020inductionAAAI,rens2020learning,DBLP:conf/kr/GiacomoFIPR20,jiang2020temporal, neary2020reward, shah2020planning, velasquez2021learning,defazio2021learning,zheng2021lifelong,camacho2021reward,corazza2022reinforcement,liu2022skill, furelos2023hierarchies, shah2024deep, zhang2023exploiting, vaezipoor2021ltl2action}. 

Critically, the use of formal languages in deep RL is nearly always predicated on knowledge of a ``ground-truth'' interpretation of the symbolic vocabulary known as a \emph{labelling function} or \emph{event detector}. This is an abstraction mapping environment states to propositional variables that is usually specified or programmed by an expert, but that can be hard to obtain in practice when dealing with high-dimensional inputs such as images. There exists a myriad of real-world settings where such an ``oracle'' is impractical and the agent must instead rely on noisy or uncertain evaluations of the vocabulary---such noise may stem from noisy sensors, partial observability, the use of neural classifiers trained from data, and so on. Under these adverse conditions, naively applying RL algorithms intended for FLs with a perfect labelling function may result in a failure to satisfy objectives or the violation of safety-critical constraints, motivating the problem we study in this work. We present the following contributions. 


\textbf{(1)} \textbf{We propose a deep RL framework for formal language reward specifications under uncertain evaluations of the vocabulary.} We specifically consider when the objective is specified as a Reward Machine (RM) \citep{icarte2018using}, which captures several FLs of interest \citep{camamacho2019ijcai}, including LTL over finite traces \citep{baier2006planning, de2013linear} and safe/co-safe fragments of LTL. We cast this problem as a POMDP, allowing us to formally characterize optimal behaviour. To our knowledge, this is the first practical deep RL framework for RMs (or similar FLs) focusing on the imperfect detection of propositions, allowing us to extend RMs to general partially observable environments. 
% \commenttk{Will the reader know what a less general case is?} \commental{is this version better?}

\textbf{(2)} \textbf{We propose and analyze a suite of RL algorithms that exploit task structure and can be deployed without a ground-truth labelling function.} We show how preexisting ``abstraction models'', noisy estimators of task-relevant features that may manifest as pretrained neural networks, sensors, heuristics, or otherwise, can be brought to bear to improve the efficiency of a learning algorithm. We use these algorithms to train agents that are aware of, and are robust to their uncertainty over the true evaluations of the vocabulary when deployed. 

\textbf{(3)} \textbf{We theoretically analyze these algorithms and their modelling assumptions.} Soundness conditions are identified for each algorithm. We discover a pitfall of naively leveraging noisy models---namely, that errors from repeated queries of a model are correlated rather than i.i.d. We show that this can have serious ramifications, including unintended or dangerous outcomes, and demonstrate how this issue can be mitigated.

\textbf{(4)} \textbf{We conduct experiments that verify our findings for noisy abstraction models trained from data.} We consider a variety of challenging domains, including domains with partial observability and high-dimensional observations. Results show that our algorithms successfully leverage task structure to improve performance while only having access to noisy interpretations of the vocabulary. 

==> sections/OLD_6-experiments.tex <==
\section{Experimental Evaluation}
\label{section:experiments}

\input{figs/env_figures}

\begin{figure*}[th!]
    \includegraphics[width=\textwidth]{figs/learning_curves.pdf}
    \vspace{-2em}
    \caption{Policy learning curves when optimizing the \emph{ground-truth} interpretation of rewards. Modelling a belief over RM states can significantly improve sample efficiency by decomposing the task, and TDM exhibits robust performance in all domains. (All results were averaged over 8 runs, with error bars showing standard error.)}
    \vspace{-0.5em}
    \label{fig:learning_curves}
\end{figure*}

We assess the proposed methods for the ARE framework in tabular and deep RL domains with 
tasks described by Reward Machines over noisy symbols. Our experiments are comprised of a series of case studies highlighting various sources of potential uncertainty in the agent's interpretation or perception of symbols. In the context of noisy symbol domains, we aim to investigate the following questions:

\vspace{-1em}
\begin{enumerate}
    \item Does exposing the task structure improve policy learning?
    \item Do the proposed methods accurately model a belief over RM states?
    \item Do the proposed methods scale to complex environments with partial observability or infinite state spaces?
\end{enumerate}

% Purposes:
% - Do the proposed methods improve performance under noisy symbols?
%     - Noise due to limited data, partial observability

% - Tasks:
%     - Predicting RM states
%     - Downstream policy learning


\subsection{Toy Grounding Models}
\label{exp:gold1}
% Purposes: 
% - do the proposed methods improve policy learning under noisy symbols?
% 
Continuing with the gold mining example under the toy belief model of gold shown in Figure~\ref{fig:gold_model}, we now train RL agents to solve the task. Our proposed methods predict a belief of having obtained gold given the trajectory observed so far, which then informs the agent's decision making. We assume here that the agent is rewarded only for executing the \emph{intended} behaviour -- that is, for obtaining \emph{real} gold and delivering it to the lab. 

\textit{\textbf{Domain.}} The environment is a $4 \times 4$ gridworld 
where the agent observes its location. Actions include moving in the four cardinal directions and a ``mine'' action. The goal is to obtain (real) gold and deliver it to the lab while minimizing movements in the grid, which incur a small cost.

\textit{\textbf{Grounding models.}} We assume that the agent can correctly identify when it's at the lab (\depot) and when it moves (\faArrows*), but cannot reliably tell whether real gold was mined (\gold).

Thresholding and IBU directly use the probabilities from the toy grounding model when evaluating \gold on each step. TDM uses these same probabilities but correctly assumes all evaluations of \gold in the same location will yield the same result -- thus, mining multiple times in a square has no effect on the belief.

\textit{\textbf{Policy Optimization.}} Each agent is implemented using Q-learning \cite{sutton2018reinforcement} with linear function approximation \cite{melo2007q} to enable generalization. In addition to the agent's location, policies are conditioned on the current belief over RM states, and a set of relevant history features to serve as memory.

\textit{\textbf{Results.}} Figure~\ref{fig:learning_curves} reports the learning curves for each method. We compared against the following baselines: a policy that observes ground-truth RM states when choosing actions (``Perfect grounding'') to set an upper limit on performance, and a memory-based policy that does not consider task structure at all (``Memory only''). Methods exploiting the task structure (Thresholding, IBU, TDM) all outperformed the ``Memory only'' baseline, despite the agent's noisy perception of the \gold symbol. TDM was more stable and sample efficient than IBU and Thresholding, with performance similar to the ``Perfect grounding'' baseline.

\subsection{Modelling RM States under Partial Observability}

We next examine whether our methods are robust to perceptual uncertainty of symbols due to partial observability. We consider two deep RL domains implemented as MiniGrid \cite{MinigridMiniworld23} environments involving image observations where key events or properties have limited observability. As before, agents are rewarded based on the ground-truth interpretation of symbols. 

\textit{\textbf{Domains.}} In the Traffic Light domain, the agent must drive along a road to pick up a package and then return home. The road has an intersection with a traffic light that periodically changes between green, yellow, and red, and the agent should not be in the intersection during a red light. However, the agent can only observe squares in front of itself. The agent's actions include moving forward and backward, waiting, and making a U-turn. An RM for this task is shown in Figure~\ref{traffic-rm} of the Appendix. 

In the Kitchen domain, a cleaning agent must enter a kitchen and make sure everything is clean: the dishes must be washed, the stove must be wiped, and the trash must be emptied. The initial condition of the kitchen may require the agent to perform any subset of these three chores (e.g. there might be no dishes to wash, but the trash and stove require the agent's attention). A positive reward is granted for pressing a button, located outside of the kitchen, only if the kitchen is in a completely clean state. However, the agent can only observe whether a chore needs to be done while inside the kitchen. The RM state for this task encodes the subset of chores that are in a clean state. 

\textit{\textbf{Grounding models.}}
For Thresholding, IBU, and TDM, the grounding models are neural networks trained online via a supervised cross-entropy loss from data collected by the agent. Thresholding and IBU train a model that predicts the values of propositions at each step, given the history, while TDM directly predicts a distribution over RM states given the history. To label the data collected by the agent, we assume access to the ground-truth labelling function $\mathcal{L}$ at \emph{training time only}. This is a reasonable assumption when training in simulation or with a sufficient number of human annotators \cite{ziegler2019fine}, but critically, execution of the policy does not depend on access to $\mathcal{L}$.

\textit{\textbf{Results.}}
Each approach was trained using PPO \cite{schulman2017proximal}, with the learning curves shown in Figure~\ref{fig:learning_curves}. In the Traffic Light domain, TDM and IBU performed near optimally, while the "Memory only" baseline and Thresholding often failed due to running the red light. We observed that the Thresholding agent would often exploit the U-turn action to drive through red lights \emph{in reverse}, allowing it to believe no red light violation occurred, as it cannot see the light colour while entering the intersection backwards.

In the Kitchen domain, TDM performed best, achieving near the maximum possible return, while Thresholding was marginally worse. IBU and the ``Memory only'' baseline made no progress. We observed that the IBU belief erroneously reflected that all chores were done without even entering the kitchen. This is because each chore has a small chance of being initialized in a clean state, and IBU incorrectly compounds this probability over time (in a similar manner to Example~\ref{example:1}). 

% \remove{The quality of the RM state beliefs produced by each approach was evaluated by measuring the log-likelihood of true RM states under random trajectories (Figure~\ref{fig:rm_belief_acc}). 
% We found that in the Traffic Light domain, IBU had the most accurate beliefs while Thresholding had the least accurate. In the Kitchen domain, TDM performed best by a wide margin. It is worth noting that the evaluation trajectories fall significantly \emph{out of distribution}, as the grounding models were trained using on-policy data.}



\subsection{Groundings Learned from Offline Data}
\label{sec:mujoco_exps}
We test the scalability of our approach on a complex MuJoCo environment involving high-dimensional observations, continuous actions, and episodes lasting thousands of steps. The task requires the agent to associate colour names with their RGB values, and we test the efficacy of grounding models trained on an offline dataset towards this task. 

\textit{\textbf{Domain.}} The agent controls a robotic car and observes lidar and RGB observations of nearby objects. Each episode, the agent must visit a specific pillar and then enter the portal, while avoiding the other pillars. The \emph{colour} (e.g. ``navy'') of the target pillar is provided at the start of each episode, and the agent must learn the association of this colour name with RGB values to reliably solve the task. The colours of the pillars and the target pillar are randomized (from a set of 18 possible colours) in each episode. 

\textit{\textbf{Grounding models.}} We collect a dataset comprised of 3.7M interactions (2K episodes) in this environment under a random policy. The data is labelled with the evaluations of propositions and RM states using the ground-truth $\mathcal{L}$. This data is then used to pretrain grounding models (expressed as neural networks) using standard supervised learning, prior to RL training.

\textit{\textbf{Results.}} Each approach was trained using PPO, with learning curves reported in Figure~\ref{fig:learning_curves}. Thresholding, IBU and TDM all exhibited performance close to the ``Perfect grounding'' baseline, while the ``Memory only'' baseline made little progress. This demonstrates that grounding models trained on offline data can provide tangible benefits to RL agents using our proposed methods. We note that these grounding models were applied in an \emph{out-of-distribution} fashion during the RL phase, as they were pretrained only on random-action trajectories. Nonetheless, our approaches were robust to this distribution shift. 

% \remove{The quality of the predicted RM state belief (evaluated under random trajectories) is reported in Figure~\ref{fig:rm_belief_acc}. The RM state beliefs predicted by TDM were more accurate compared to Thresholding and IBU.}



\subsection{Accuracy of Predicted RM Beliefs}

For each of the domains in Sections~\ref{exp:gold1} - \ref{sec:mujoco_exps}, we compare Thresholding, IBU, and TDM in terms of accuracy of the predicted RM state belief. Grounding models are neural networks trained on datasets comprised of 2K episodes labelled with ground-truth evaluations of propositions and RM states, under a random-action policy. Validation and test datasets (100 episodes, each) are used for hyperparameter selection and evaluation, respectively.

\begin{figure}
    \hspace{-0.95em}\includegraphics[width=1.1\columnwidth]{figs/bar.pdf}
    \vspace{-2em}
    
    \caption{Accuracy of RM state prediction methods measured by log-likelihood (higher is better) of the true RM state given the history across the test dataset. TDM predicts the RM state belief more accurately than Thresholding and IBU. (All results were averaged over 8 runs, with error lines showing standard error.)}
    \label{fig:rm_belief_acc}
\end{figure}

\textbf{\textit{Results.}} Figure~\ref{fig:rm_belief_acc} reports the accuracy of each approach in terms of log-likelihood across the test dataset. For Thresholding and IBU, we substituted likelihoods of $0$ with $0.01$. The RM state beliefs produced by TDM are significantly more accurate than Thresholding and IBU. 








\subsection{RL with an Internal Reward Model}
\label{exp:gold2}
We explore the prospect of training an RL agent without requiring explicit feedback from the environment in the form of rewards. Instead, we leverage the agent's belief over RM states to optimize the agent's \emph{perceived rewards}. Optimizing a proxy objective is known to be challenging in RL \cite{lambert2023alignment}, and our key question is whether noisy grounding models can serve as a reliable proxy to learn the desired behaviour. 

We adopt the same setup as in the previous gold mining experiment, except the agent no longer receives rewards based on whether \emph{actual} gold was obtained upon reaching the lab. Instead, the agent optimizes its expected \emph{belief} of having obtained gold and then visiting the lab. 

% \begin{figure*}
%     \centering

%     \begin{subfigure}[t]{0.40\textwidth}
%         \centering
%         \includegraphics[width=0.94\textwidth]{figs/internal_rewards.pdf}
%         \caption{Final performance of an agent optimizing predicted rewards under an RM state belief. We report the agent's actual return vs its predicted returns, averaged over 100 episodes $\times$ 8 training runs. Thresholding and IBU exhibited overfitting to erroneous reward predictions.}
%         \vspace{-1em}
%         \label{fig:perceived}
%     \end{subfigure}
%     \hspace{1em}
%     \begin{subfigure}[t]{0.57\textwidth}
%         \hspace{-2em}\includegraphics[width=1.15\textwidth]{figs/rm_belief_acc.pdf}
%         \caption{Accuracy of RM state beliefs predicted by each method. We evaluated the log-likehood of the ground-truth RM state averaged over 100 random-action episodes and all possible histories within those episodes, with error lines showing standard error.}
%         \label{fig:rm_belief_acc}
%     \end{subfigure}

% \end{figure*}


\begin{figure}
    \centering
    \includegraphics[width=0.94\columnwidth]{figs/internal_rewards.pdf}
    \caption{The agent's actual vs perceived performance when optimizing perceived rewards given by its RM state belief. Results are averaged over 8 runs, with error bars showing standard error. TDM is robust to noisy symbols, allowing the agent to produce the desired behaviour \emph{without} ground-truth rewards. Thresholding and IBU diverge from the desired behaviour and overfit to the proxy rewards.}
    \vspace{-1em}
    \label{fig:perceived}
    % \begin{minipage}[t]{0.40\textwidth}
    %     \centering

    % \end{minipage}
    % \hspace{1em}
    % \begin{minipage}[t]{0.57\textwidth}
    %     \hspace{-2em}\includegraphics[width=1.15\textwidth]{figs/rm_belief_acc.pdf}
    %     \caption{Accuracy of RM state beliefs predicted by each method. We evaluated the log-likehood of the ground-truth RM state averaged over 100 random-action episodes and all possible histories within those episodes, with error lines showing standard error.}
    %     \label{fig:rm_belief_acc}
    % \end{minipage}

\end{figure}

\textit{\textbf{Results.}} 
Figure~\ref{fig:perceived} reports the agent's \emph{actual} returns (the desired objective) vs its \emph{perceived} returns (the proxy objective) over the course of training. When updating the RM state belief with TDM, both the actual and perceived returns were high, suggesting that TDM can yield a reliable proxy under noisy symbols. On the other hand, IBU and Thresholding led to a disconnect between perceived and actual returns, resulting in poor performance on the desired objective.

Qualitatively, we observed the following behaviours. The Thresholding agent visited the closer fool's gold location that is incorrectly believed to be gold with $60\%$ probability, then immediately headed to the lab. IBU consistently mined at the same fool's gold location several times before returning to the lab. In contrast, TDM adopted the robust strategy of mining at several different locations to maximize the probability of obtaining gold. 
